Degradation-Aware Image Enhancement via Vision-Language Classification

Image degradation is a prevalent issue in various real-world applications, affecting visual quality and downstream processing tasks. In this study, we propose a novel framework that employs a Vision-Language Model (VLM) to automatically classify degraded images into predefined categories. The VLM categorizes an input image into one of four degradation types: (A) super-resolution degradation (including noise, blur, and JPEG compression), (B) reflection artifacts, (C) motion blur, or (D) no visible degradation (high-quality image). Once classified, images assigned to categories A, B, or C undergo targeted restoration using dedicated models tailored for each specific degradation type. The final output is a restored image with improved visual quality. Experimental results demonstrate the effectiveness of our approach in accurately classifying image degradations and enhancing image quality through specialized restoration models. Our method presents a scalable and automated solution for real-world image enhancement tasks, leveraging the capabilities of VLMs in conjunction with state-of-the-art restoration techniques.

==> Tables/table1.tex <==
\begin{table*}[htbp]
    \centering
    \caption{Evaluation Scores of Text-to-Image Models}
    \label{tab:eval_scores}
    \begin{tabular}{|l|c|c|c|c|}
        \hline
        \textbf{Model} & \textbf{Image} & \textbf{Prompt Adherence} & \textbf{Coherence and Consistency} & \textbf{Visual Fidelity and Aesthetics} \\
        \hline
        \multirow{11}{*}{Stable Diffusion XL (SDXL)} & Image 1 & 4.2 & 4.1 & 4.5 \\
        \cline{2-5}
        & Image 2 & 4.3 & 4.0 & 4.4 \\
        \cline{2-5}
        & Image 3 & 4.1 & 4.2 & 4.3 \\
        \cline{2-5}
        & Image 4 & 4.0 & 3.9 & 4.2 \\
        \cline{2-5}
        & Image 5 & 4.5 & 4.3 & 4.6 \\
        \cline{2-5}
        & Image 6 & 4.2 & 4.1 & 4.5 \\
        \cline{2-5}
        & Image 7 & 4.3 & 4.0 & 4.4 \\
        \cline{2-5}
        & Image 8 & 4.1 & 4.2 & 4.3 \\
        \cline{2-5}
        & Image 9 & 4.0 & 3.9 & 4.2 \\
        \cline{2-5}
        & Image 10 & 4.4 & 4.4 & 4.7 \\
        \cline{2-5}
        & \textbf{Average} & 4.2 & 4.1 & 4.4 \\
        \hline
        \multirow{11}{*}{Stable Diffusion 3.5 (SD3.5)} & Image 1 & 3.8 & 3.7 & 3.9 \\
        \cline{2-5}
        & Image 2 & 3.9 & 3.8 & 4.0 \\
        \cline{2-5}
        & Image 3 & 3.7 & 3.6 & 3.8 \\
        \cline{2-5}
        & Image 4 & 3.8 & 3.7 & 3.9 \\
        \cline{2-5}
        & Image 5 & 4.0 & 3.9 & 4.1 \\
        \cline{2-5}
        & Image 6 & 3.9 & 3.8 & 4.0 \\
        \cline{2-5}
        & Image 7 & 3.8 & 3.7 & 3.9 \\
        \cline{2-5}
        & Image 8 & 3.7 & 3.6 & 3.8 \\
        \cline{2-5}
        & Image 9 & 3.8 & 3.7 & 3.9 \\
        \cline{2-5}
        & Image 10 & 4.1 & 4.0 & 4.2 \\
        \cline{2-5}
        & \textbf{Average} & 3.8 & 3.7 & 3.9 \\
        \hline
        \multirow{11}{*}{FLUX} & Image 1 & 4.0 & 3.9 & 4.2 \\
        \cline{2-5}
        & Image 2 & 4.1 & 4.0 & 4.3 \\
        \cline{2-5}
        & Image 3 & 3.9 & 3.8 & 4.1 \\
        \cline{2-5}
        & Image 4 & 4.0 & 3.9 & 4.2 \\
        \cline{2-5}
        & Image 5 & 4.2 & 4.1 & 4.4 \\
        \cline{2-5}
        & Image 6 & 4.1 & 4.0 & 4.3 \\
        \cline{2-5}
        & Image 7 & 4.0 & 3.9 & 4.2 \\
        \cline{2-5}
        & Image 8 & 3.9 & 3.8 & 4.1 \\
        \cline{2-5}
        & Image 9 & 4.0 & 3.9 & 4.2 \\
        \cline{2-5}
        & Image 10 & 4.3 & 4.2 & 4.5 \\
        \cline{2-5}
        & \textbf{Average} & 4.0 & 3.9 & 4.2 \\
        \hline
    \end{tabular}
\end{table*}
